Ethereal: Divide and Conquer Network Load Balancing in Large-Scale Distributed Training

Large-scale distributed training in production datacenters constitutes a challenging workload bottlenecked by network communication. In response, both major industry players (e.g., Ultra Ethernet Consortium) and parts of academia have surprisingly, and almost unanimously, agreed that packet spraying is \emph{necessary} to improve the performance of large-scale distributed training workloads. In this paper, we challenge this prevailing belief and pose the question: \emph{How close can singlepath transport come to matching the performance of packet spraying?} We demonstrate that singlepath transport (from a NIC's perspective) is sufficient and can perform nearly as well as ideal packet spraying, particularly in the context of distributed training in CLOS-based topologies. Our assertion is based on four key observations about workloads driven by collective communication patterns: \emph{(i)} flow sizes are known upon arrival, \emph{(ii)} flow sizes are equal within each step of a collective, \emph{(iii)} the completion time of a collective is more critical than individual flow completion times, and \emph{(iv)} flows can be \emph{split} upon arrival to control load balancing directly from the application layer. We present Ethereal, a simple distributed load balancing algorithm that opportunistically splits flows and assigns paths to each flow in a transparent manner, requiring little to no changes to existing RDMA NICs. Our evaluation, spanning a wide range of collective communication algorithms and GPT models using Astra-Sim, shows that Ethereal significantly reduces the completion times by up to $30\%$ compared to packet spraying and by up to $40\%$ compared to REPS, even under link failures. This paper offers an alternative perspective for developing next-generation transport protocols tailored to large-scale distributed training.

==> macros.tex <==
%!TEX ROOT = main.tex
\usepackage{enumitem}

\makeatletter
 \renewcommand\subsubsection{\@startsection {subsubsection}{3}{\z@}%
     {-2.5ex \@plus -1ex \@minus -.2ex}%
     {1.3ex \@plus.2ex}%
    {\ACM@NRadjust\@subsubsecfont}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%     {-.75\baselineskip \@plus -.2\p@ \@minus -.2\p@}% before \@plus -2\p@ <<<
%     {.25\baselineskip}%
%     {\ACM@NRadjust\@secfont}}
% \@startsection {NAME}{LEVEL}{INDENT}{BEFORESKIP}{AFTERSKIP}{STYLE} 
%            optional * [ALTHEADING]{HEADING}
%    Generic command to start a section.  
%    NAME       : e.g., 'subsection'
%    LEVEL      : a number, denoting depth of section -- e.g., chapter=1,
%                 section = 2, etc.  A section number will be printed if
%                 and only if LEVEL gt or eq the value of the secnumdepth
%                 counter.
%    INDENT     : Indentation of heading from left margin
%    BEFORESKIP : Absolute value = skip to leave above the heading.  
%                 If negative, then paragraph indent of text following 
%                 heading is suppressed.
%    AFTERSKIP  : if positive, then skip to leave below heading,
%                       else - skip to leave to right of run-in heading.
%    STYLE      : commands to set style
%  If '*' missing, then increments the counter.  If it is present, then
%  there should be no [ALTHEADING] argument.  A sectioning command
%  is normally defined to \@startsection + its first six arguments.
\makeatother

% Colors
\definecolor{darkgreen}{rgb}{0.01, 0.75, 0.24}
\definecolor{darkcyan}{rgb}{0.0, 0.55, 0.55}
\definecolor{mycolor}{rgb}{0.01, 0.75, 0.24}
\definecolor{takeawaycolor}{rgb}{0.75, 0, 0}
\definecolor{mygray}{gray}{0.9}
\definecolor{myred}{rgb}{0.75, 0, 0}
\definecolor{alg1}{rgb}{0.898, 1, 0.914}
\definecolor{alg2}{rgb}{0.925, 0.988, 1}
\definecolor{alg3}{rgb}{1, 1, 0.906}
\definecolor{alg4}{rgb}{1, 0.922, 0.922}
% hypen
\mathchardef\hyphen="2D

% Formal
\newtheoremstyle{sltheorem}
{}                % Space above
{}                % Space below
{\slshape}        % Theorem body font % (default is "\upshape")
{}                % Indent amount
{\bfseries}       % Theorem head font % (default is \mdseries)
{.}               % Punctuation after theorem head % default: no punctuation
{ }               % Space after theorem head
{}                % Theorem head spec
\theoremstyle{sltheorem}
% \theoremstyle{plain}
\newtheorem{prop}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}
\newtheorem{observation}{Observation}
\newtheorem{condition}{Condition}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{Lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{property}{Property}
\newtheorem{heuristic}{Heuristic}

% For custom bold heading
\newcommand{\myitem}[1]{\vspace{1mm}\noindent\textbf{#1}}
\newcommand{\myitemit}[1]{\noindent\textit{#1}}
% \makeatletter\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}{3.25ex \@plus1ex \@minus.2ex}{-1em}{\normalfont\normalsize\itshape}}\makeatother

\newcommand{\remove}[1]{}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

% Some shortcuts for text
\newcommand{\first}{\emph{(i)}\xspace}
\newcommand{\second}{\emph{(ii)}\xspace}
\newcommand{\third}{\emph{(iii)}\xspace}
\newcommand{\fourth}{\emph{(iv)}\xspace}
\newcommand{\fifth}{\emph{(v)}\xspace}
\newcommand{\sixth}{\emph{(vi)}\xspace}
\newcommand{\seventh}{\emph{(vii)}\xspace}
\usepackage{xcolor}
\definecolor{light-gray}{gray}{0.9}
\usepackage{tcolorbox}
% \usepackage{soul}
% \newcommand{\mathcolorbox}[2]{\colorbox{#1}{$\displaystyle #2$}}


\newcommand{\First}{\emph{(I)}\xspace}
\newcommand{\Second}{\emph{(II)}\xspace}
\newcommand{\Third}{\emph{(III)}\xspace}
\newcommand{\Fourth}{\emph{(IV)}\xspace}
\newcommand{\Fifth}{\emph{(V)}\xspace}
\newcommand{\Sixth}{\emph{(VI)}\xspace}
\newcommand{\Seventh}{\emph{(VII)}\xspace}

\newcommand{\ie}{i.e., \@}
\newcommand{\eg}{e.g., \@}
\newcommand{\etc}{etc., \@}
\newcommand{\etal}{et al.\xspace}

\newcommand{\xref}[1]{\S\ref{#1}}
\newcommand{\axref}[1]{Appendix~\ref{#1}}
\newcommand{\cref}[1]{Chapter~\ref{#1}}
\newcommand{\pxref}[1]{(\xref{#1})}
\newcommand{\fref}[1]{Fig.~\ref{#1}}
\newcommand{\tref}[1]{Table~\ref{#1}}
